Reformulating $\epsilon$-$\delta$ Limits in a Pedagogically Cleaner Way

We provide a simple reformulation of the $\epsilon$-$\delta$ limit definition introduced in undergraduate calculus courses that enhances its pedagogical value for conceptual understanding and computational skill.

==> Credits.tex <==
\usepackage{fancyhdr}
\pagestyle{fancy}
\renewcommand{\headrulewidth}{0pt}
\fancyhf{}
\fancyfoot[C]{\textsc{KindiakMath Notes}}
\fancyfoot[LE,RO]{\thepage}

==> contact.tex <==
Contact info:
\begin{itemize}
	\item Name: Joel Chang
	\item Contact: \href{mailto:joel.chang@u.nus.edu}{joel.chang@u.nus.edu}
	\item Consultation Hours: Wednesday, 10am--12pm
\end{itemize}

\newpage

\begin{center}
\underline{Q\&A}
\end{center}

==> details.tex <==
\renewcommand{\modulename}{MA2002 Calculus}
\renewcommand{\tutnumber}{1}
\renewcommand{\tutorialheader}{Tutorial \tutnumber\ Summary}
\renewcommand{\semester}{Semester 1, 2022/2023}

==> qraw.tex <==
\begin{flushleft}
Just a quick introduction of myself:
\begin{itemize}
	\item Name: Joel Chang
	\item Contact: \href{mailto:joel.chang@u.nus.edu}{joel.chang@u.nus.edu}
	\item Consultation Hours: Wednesday, 10am--12pm
	\item H/P, Instagram, Wordpress (aka chill, non-tutor Joel): End of the module
\end{itemize}
About me:
\begin{itemize}
	\item Year 3 Mathematics Major
	\item Really enjoys learning mathematics
	\item A Christian who conducts monthly bible studies with several groups of friends
	\item Otherwise, pretty boring person
	\item Let's do math!
\end{itemize}
\end{flushleft}

{\color{\mytablecolor} \hrule}
%\newpage
\begin{center}
Primary questions for discussion: 2, 6, 8, 9, 10b
\end{center}

\begin{enumerate}
	\addtocounter{enumi}{1}
	\item \easy Simplify the propositions below using the laws given in \textbf{Theorem 2.1.1 (Epp)} and the implication law (if necessary) with only negation ($\neg$), conjunction ($\wedge$) and disjunction ($\lor$) in your final answers. \warn{Supply a justification for every step.}
	\begin{enumerate}
	\item $\neg a \wedge (\neg a \to (a \wedge b))$
	
	Raflee worked out his answer as shown below. However, he skipped some steps and hence his answer will not be awarded full credit. Can you point out the omissions?
	\begin{align*}
	&\neg a \wedge (\neg a \to (a \wedge b))\\
	&\equiv {\neg a} \wedge (a \lor (a \wedge b)) && \text{(implication law)}\\
	&\equiv {\neg a} \wedge a &&\text{(absorption law)} &&\\
	&\equiv \mathbf{false} && \text{(negation law)}
	\end{align*}
	\vfill \newpage
	\item $(p \lor {\neg q}) \to q$
	\vfill
	
	\item $\neg(p \lor {\neg q}) \lor ({\neg p} \wedge {\neg q})$
	\vfill
	\item $(p \to q) \to r$
	\vfill
	\end{enumerate}\newpage
	\addtocounter{enumi}{3}
	\item \medium Some of the arguments below are valid, whereas others exhibit the converse or inverse error. Use symbols to write the logical form of each argument. If the argument is valid, identify the rule of inference that guarantees its validity. Otherwise, state whether the converse or the inverse error is made.
	\begin{enumerate}
	\item \warn{Sandra knows Java and Sandra knows C++.
	
	$\therefore$ Sandra knows C++.}
	
	Let $p = \text{``Sandra knows Java''}$.
	
	Let $q = \text{``Sandra knows C++''}$.
	\vfill
	
	\item \warn{If at least one of these two numbers is divisible by $6$, then the product of these two numbers is divisible by $6$.
	
Neither of these two numbers is divisible by $6$.

$\therefore$ The product of these two numbers is not divisible by $6$.}

	Let $p = \text{``The first number is divisible by $6$''}$.
	
	Let $q = \text{``The second number is divisible by $6$''}$.
	
	Let $r = \text{``The product of these two numbers is divisible by $6$''}$.
\vfill\newpage
	\item \warn{If there are as many rational numbers as there are irrational numbers, then the set of all irrational numbers is infinite.
	
The set of all irrational numbers is infinite.

	$\therefore$ There are as many rational numbers as there are irrational numbers.}
	
	Let $p = \text{``There are as many rational numbers as there are irrational numbers''}$.
	
	Let $q = \text{``The set of all irrational numbers is infinite''}$.
	\vfill 
	\item \warn{If I get a Christmas bonus, I'll buy a stereo.
If I sell my motorcycle, I'll buy a stereo.

$\therefore$ If I get a Christmas bonus or I sell my motorcycle, I'll buy a stereo.}

	Let $p = \text{``I get a Christmas bonus''}$.
	
	Let $q = \text{``I sell my motorcycle''}$.
	
	Let $r = \text{``I'll buy a stereo''}$.
\vfill
	\end{enumerate}
	\addtocounter{enumi}{1}\newpage
	\item[8b.] \medium The island of Wantuutrewan is inhabited by two types of people: knights who always tell the truth and knaves who always lie. You visit the island and have the following encounters with the natives.
	
	Two natives $C$ and $D$ speak to you:
	\begin{itemize}[label={}]
		\item $C$ says: $D$ is a knave.
		\item $D$ says: $C$ is a knave.
	\end{itemize}
	How many knights and knaves are there? \vfill
	\addtocounter{enumi}{1}\newpage
	\item \medium Prove Tutorial \#1 Lemma \#1:
The product of any two odd integers is an odd integer. \vfill
	\item[10b.] \hard Your classmate Smart came across this question:
$$\text{If $a,b,c$ are integers such that $a^2+b^2=c^2$, then $a,b$ cannot both be odd.}$$

Write your own proof using contraposition. You may start your proof with the same line $1$ as above. You may also make use of Lemma 1 in the previous question.
\vfill
\end{enumerate}

==> raw.tex <==
\begin{definition}
	TBC
\end{definition}
\begin{theorem}
	TBC	
\end{theorem}

